EquiformerV2: Improved Equivariant Transformer for Scaling to Higher-Degree Representations

Equivariant Transformers such as Equiformer have demonstrated the efficacy of applying Transformers to the domain of 3D atomistic systems. However, they are limited to small degrees of equivariant representations due to their computational complexity. In this paper, we investigate whether these architectures can scale well to higher degrees. Starting from Equiformer, we first replace $SO(3)$ convolutions with eSCN convolutions to efficiently incorporate higher-degree tensors. Then, to better leverage the power of higher degrees, we propose three architectural improvements -- attention re-normalization, separable $S^2$ activation and separable layer normalization. Putting this all together, we propose EquiformerV2, which outperforms previous state-of-the-art methods on large-scale OC20 dataset by up to $9\%$ on forces, $4\%$ on energies, offers better speed-accuracy trade-offs, and $2\times$ reduction in DFT calculations needed for computing adsorption energies. Additionally, EquiformerV2 trained on only OC22 dataset outperforms GemNet-OC trained on both OC20 and OC22 datasets, achieving much better data efficiency. Finally, we compare EquiformerV2 with Equiformer on QM9 and OC20 S2EF-2M datasets to better understand the performance gain brought by higher degrees.

==> content/2_3_irreducible_representations.tex <==
\vspace{-2.5mm}
\subsection{Irreducible Representations}
\vspace{-2.5mm}
\label{subsec:irreducible_representations}
%A powerful result of group representation theory is that the action of group elements can be expressed as matrices acting on vector spaces via matrix multiplication. Colloquially, we use the term ``representation'' to refer to both the vector space and the representation of the group as matrices acting on that vector space.
%A group representation defines how we write down transformation matrices of group elements that act on a vector space. Equivariant operations commute with the action of the group on the vector space.
%\todo{[Cite group representation theory.]}
A group representation~\citep{Dresselhaus2007, zee} defines transformation matrices $D_{X}(g)$ of group elements $g$ that act on a vector space $X$. 
%Equivariant operations commute with the action of the group on the vector space.
For 3D Euclidean group $E(3)$, two examples of vector spaces with different transformation matrices are scalars and Euclidean vectors in $\mathbb{R}^3$, i.e., vectors change with rotation while scalars do not.
%\tess{In this work, we only consider relative positions (similar to convolutions) and do not need to directly treat the group of translation $T(3)$. However, we must address $O(3)$ which is the direct product of 3D rotations $SO(3)$ and inversion $\mathbb{Z}_2$.
%The transformation matrices of rotation and inversion are separable and commute, so we first focus on the irreducible representations of $SO(3)$.}
%To address translation symmetry, we simply operate on relative positions; below we focus our discussion on $O(3)$ which requires a more complex treatment.
To address translation symmetry, we operate on relative positions.
%%%Below we focus our discussion on $O(3)$.
% Since we only operate on relative positions, we do not consider translation but only focus on $O(3)$.
%The transformation matrices of rotation and inversion are separable and commute, so we first focus on the irreducible representations of $SO(3)$.
%%%The transformation matrices of rotation and inversion are separable and commute, and we first discuss irreducible representations of $SO(3)$.
The transformation matrices of rotation and inversion are separable and commute. 
%%%We discuss irreducible representations of $SO(3)$ below and those of inversion in appendix \todo{Section of inversion}.
We discuss irreducible representations of $SO(3)$ below and discuss inversion in Sec.~\ref{appendix:subsec:equivariant_irreps_feature} in appendix.
%There are many ways to represent a group. If there exists a change of basis $P$ for a given representation $D(g)$ such that $P^{-1} D(g) P = D'(g)$ that makes $D'(g)$ block diagonal for all $g \in G$, meaning $g$ acts on independent subspaces of the vector space, the representation $D(g)$ is deemed reducible. A particular class of representations that are convenient for generalizable, composable functions are irreducible representations or ``irreps'', which cannot be further reduced. We can express any group representation as a direct sum of irreps \cite{zee,Dresselhaus2007,e3nn}. 

%Since we only consider relative positions, we can ignore translation and focus on a smaller group of rotation and inversion called $O(3)$ contained in $E(3)$. 
%$O(3)$ is the direct product of $SO(3) \times \mathbb{Z}_2$, where $\mathbb{Z}_2$ is the inversion group (the group of 1 and -1), so we can deal with the irreps of these two groups separately. 

%\tess{Any group representation of $SO(3)$ on a given vector space can be decomposed into a direct sum (concatenation) of provably smallest transformation matrices called irreducible representations (irreps).}
%Any group representation of $SO(3)$ on a given vector space can be decomposed into a direct sum (concatenation) of provably smallest transformation matrices called irreducible representations (irreps).
Any group representation of $SO(3)$ on a given vector space can be decomposed into a concatenation of provably smallest transformation matrices called irreducible representations (irreps).
Specifically, for group element $g \in SO(3)$, there are $(2L+1)$-by-$(2L+1)$ irreps matrices $D_{L}(g)$ called Wigner-D matrices acting on $(2L+1)$-dimensional vector spaces, where degree $L$ is a non-negative integer.
$L$ can be interpreted as an angular frequency and determines how quickly vectors change when rotating coordinate systems.
$D_{L}(g)$ of different $L$ act on independent vector spaces.
Vectors transformed by $D_{L}(g)$ are type-$L$ vectors, with scalars and Euclidean vectors being type-$0$ and type-$1$ vectors.
%\revision{It is common to index these $(2L+1)$ dimensions with an index $m$ called order, where $-L \leq m \leq L$.}
It is common to index elements of type-$L$ vectors with an index $m$ called order, where $-L \leq m \leq L$.

%The inversion group which is isomorphic $\mathbb{Z}_2$ has two elements, the identity and inversion, commonly notated as 1 and -1, and only two irreps: one even ($e$) irrep that does not change sign under inversion and an odd irrep which does. We create irreps of $O(3)$ by simply multiplying $SO(3)$ and $\mathbb{Z}_2$ irreps.
%\revision{The group of inversion $\mathbb{Z}_2$ only has two elements, identity and inversion denoted as $1$ and $-1$, and therefore only two irreps, even $e$ and odd $o$.}

\begin{comment}
\todo{The group of inversion $\mathbb{Z}_2$ only has two elements, identity and inversion, and two irreps, even $e$ and odd $o$.
Vectors transformed by irrep $e$ do not change sign under inversion while those by irrep $o$ do.
We create irreps of $O(3)$ by simply multiplying those of $SO(3)$ and $\mathbb{Z}_2$,  and we introduce parity $p$ to type-$L$ vectors to denote how they transform under inversion.
%Therefore for $O(3)$, type-$L$ vectors in $SO(3)$ are extended to type-$(L, p)$ vectors, where $p$ is $e$ or $o$.
Therefore, type-$L$ vectors in $SO(3)$ are extended to type-$(L, p)$ vectors in $O(3)$, where $p$ is $e$ or $o$.
In the following, we use type-$L$ vectors for the ease of discussion, but we can generalize to type-$(L, p)$ vectors, unless otherwise stated.}
\end{comment}

\vspace{-3mm}
\paragraph{Irreps Features.}
We concatenate multiple type-$L$ vectors to form $SE(3)$-equivariant irreps features. 
%We additionally index our type-$L$ features by parity $p$ which indicates the whether the feature is even or odd under inversion, but for simplicity we drop this index from our description.
Concretely, irreps feature $f$ has $C_{L}$ type-$L$ vectors, where $0 \leq L \leq L_{max}$ and $C_{L}$ is the number of channels for type-$L$ vectors.
%\tess{We index irreps features $f$ by channel $c$, degree $L$, order $m$, and parity $p$ and denote as $f^{(L, p)}_{c, m}$.}
We index irreps features $f$ by channel $c$, degree $L$, and order $m$ and denote as $f^{(L)}_{c, m}$.
%\revision{Different channels of type-$L$ vectors are parametrized by different weights but are transformed with the same Wigner-D matrix $D_{L, p}(g)$.}
Different channels of type-$L$ vectors are parametrized by different weights but are transformed with the same $D_{L}(g)$.
%\tess{}{Note that regular scalar features correspond to including only type-$0$ vectors with even parity with $D_{0, \text{even}}(g)$ being identity for all $g$.}
Regular scalar features correspond to only type-$0$ vectors.
%Note that this can generalize to include inversion by extending $L$ to $(L, p)$.
%This can generalize to $E(3)$ by including inversion and extending $L$ to $(L, p)$.

\vspace{-3mm}
\paragraph{Spherical Harmonics.}
Euclidean vectors $\vec{r}$ in $\mathbb{R}^3$ can be projected into type-$L$ vectors $f^{(L)}$ by using spherical harmonics (SH) $Y^{(L)}$: $f^{(L)} = Y^{(L)}(\frac{\vec{r}}{|| \vec{r} ||})$.
SH are $E(3)$-equivariant with $D_L(g) f^{(L)} = Y^{(L)}(\frac{D_{1}(g) \vec{r}}{|| D_{1}(g) \vec{r} ||})$.
SH of relative position $\vec{r}_{ij}$ generates the first set of irreps features. Equivariant information propagates to other irreps features through equivariant operations like tensor products.


% The irreducible matrix representations of $g \in SO(3)$ are called the Wigner-D matrices, $D_{L}(g)$. These $(2L+1)$-by-$(2L+1)$ transformation matrices act on $(2L+1)$-dimensional vectors, with $L$, a positive integer inclusive of zero, corresponding to the degree of the irrep, which can be interpreted as an angular frequency i.e. how quickly the feature changes under a rotation of the coordinate system. It is common to index these $(2L+1)$ dimensions with an additional index $m$ called the order where $-L \leq m \leq L$. There are only 2 irreps of the inversion group and they are both 1-dimensional; they correspond to whether or not something changes sign under spatial inversion $(x, y, z) = (-x, -y, -z)$. $D(g) = 1, \forall g \in \mathbb{Z}_2$ for the even irrep and $D(i) = -1$ for the odd irrep, where $i$ indicates the inversion operation.

% We use the irreps of $O(3)$ to express features, which define how these features transform under rotation and inversion (or parity). The irreps of $O(3)$ are identified by two values: the angular frequency $L$ from the irreps of $O(3)$ and the parity $p$ which is even (1) or odd (-1) from the irreps of inversion or $\mathbb{Z}_2$. For example, a scalar like a mass or atom type does not change under rotation and it does not change under spatial inversion, thus it is denoted as $L=0, p=1$ or ``even''. A vector like a force or a position rotates at the same frequency as a rotation of the coordinate system and does incur a minus sign under inversion, thus it is denoted as $L=1, p=-1$ or ``odd''. In \texttt{e3nn}, scalars and vectors are notated as \texttt{0e} and \texttt{1o}, respectively. 

% \paragraph{Irrep Features.}
% We express the vector spaces of equivariant features as a direct sum of irrep vector spaces. This direct sum can contain multiple copies of a given irrep. For example, if our features contain one scalar and two vectors, we say the features transform as the direct sum of one scalar irrep and two vector irreps; in \texttt{e3nn} we use \texttt{o3.Irreps('1x0e+2x1o')} to denote this where the format \texttt{cxLp} means \texttt{c} copies or channels of the irrep with $L$ and $p$. We use the term irrep features to denote features that span a vector space composed of a direct sum of irrep vector spaces.

% Because irreps have different sizes, in practice we concatenate our direct sum of irrep vector spaces along the feature dimension and keep track which specific irrep each element in the feature vector corresponds to; in \texttt{e3nn} this is taken care of by the \texttt{o3.Irreps} class. Thus, the dimensionality of a given instance of irrep features is equal to $sum_{L \in \text{irreps}} c \times (2 L + 1)$. In the case of multiple copies of a given irrep in a given irrep features, each irrep of the same type are parameterized by different weights but under rotation are transformed with the same Wigner-D matrix. 

% We index irreps features $f$ by channel $c$, degree $l$, and order $m$ and denote as $f^{(l)}_{c, m}$. Note that regular scalar features corresponds to including only type-$0$ vectors.

%\todo{Add the reason to incorporate vectors of higher $l$}

%\paragraph{Projecting 3D Vectors onto Spherical Harmonics.}
%Euclidean vectors $\vec{r}$ in $\mathbb{R}^3$ can be projected into type-$l$ vectors $f^{(l)}$ by using spherical harmonics $Y^{(l)}$: $f^{(l)} = Y^{(l)}(\frac{\vec{r}}{|| \vec{r} ||})$.
%The spherical harmonics embedding of relative position $\vec{r}_{ij}$ generates the first set of equivariant irreps features that we use in our network.

%\todo{Add a figure showing spherical harmonic projection}

==> content/2_4_tensor_product.tex <==
\vspace{-2.5mm}
\subsection{Tensor Product}
\label{subsec:tensor_product}
\vspace{-2.5mm}
%We use the tensor product to interact vectors of different irreps features. 
%%%We use tensor products to interact different type-$L$ vectors and first discuss the tensor product for $SO(3)$.
Tensor products can interact different type-$L$ vectors.
We discuss tensor products for $SO(3)$ below and those for $O(3)$ in Sec.~\ref{appendix:subsec:tensor_product}.
%We first discuss the tensor product for $SO(3)$.
The tensor product denoted as $\otimes$ uses Clebsch-Gordan coefficients to combine type-$L_1$ vector $f^{(L_1)}$ and type-$L_2$ vector $g^{(L_2)}$ and produces type-$L_3$ vector $h^{(L_3)}$:
\begin{equation}
h^{(L_3)}_{m_3} = (f^{(L_1)} \otimes g^{(L_2)})_{m_3} = \sum_{m_1 = -L_1}^{L_1} \sum_{m_2 = -L_2}^{L_2} C^{(L_3, m_3)}_{(L_1, m_1)(L_2, m_2)} f^{(L_1)}_{m_1} g^{(L_2)}_{m_2} 
\label{eq:tensor_product}
\end{equation}
where $m_1$ denotes order and refers to the $m_1$-th element of $f^{(L_1)}$.
Clebsch-Gordan coefficients $C^{(L_3, m_3)}_{(L_1, m_1)(L_2, m_2)}$ are non-zero only when $| L_1 - L_2 | \leq L_3 \leq | L_1 + L_2 |$ and thus restrict output vectors to be of certain types.
For efficiency, we discard vectors with $L > L_{max}$, where $L_{max}$ is a hyper-parameter, to prevent vectors of increasingly higher dimensions.
%%%The tensor product is an equivariant operation, with $ ( D_{L_1}(g') f^{(L_1)} ) \otimes ( D_{L_2}(g') g^{(L_2)} ) = D_{L_3}(g') h^{(L_3)} $ for $g' \in SO(3)$.

%To make our tensor product additionally preserve inversion symmetry, we simply keep track of the output parity using the following multiplication rules: \tess{$e \times e = e$, $o \times o = e$, and $e \times o = o \times e = o$}.


%\paragraph{Incorporating Learnable Weights.}
%\tess{We call each distinct nontrivial combination of $L_1 p_1 \otimes L_2 p_2 \rightarrow L_3 p_3$ a path.}
%\tess{For example, a type-$1o$ vector tensor producted with another type-$1o$ vector gives rise to vectors of type $0e$, $1e$ and $2e$ and therefore $3$ paths.}
We call each distinct non-trivial combination of $L_1 \otimes L_2 \rightarrow L_3$ a path.
%\tess{For example, a type-$1o$ vector tensor producted with another type-$1o$ vector gives rise to vectors of type $0e$, $1e$ and $2e$ and therefore $3$ paths.}
Each path is independently equivariant, and we can assign one learnable weight to each path in tensor products, which is similar to typical linear layers.
We can generalize Eq.~\ref{eq:tensor_product} to irreps features and include multiple channels of vectors of different types through iterating over all paths associated with channels of vectors.
In this way, weights are indexed by $(c_1, l_1, c_2, l_2, c_3, l_3)$, where $c_1$ is the $c_1$-th channel of type-$l_1$ vector in input irreps feature.
We use $\otimes_{w}$ to represent tensor product with weights $w$. % and denote tensor product of two irreps features $f_1$ and $f_2$ as $f_1 \otimes _w f_2$.
Weights can be conditioned on quantities like relative distances.
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%For example, in GNNs, we use tensor products of irreps features $f_j$ and SH embedding of relative position $\vec{r}_{ij}$ to transform features into messages and use some learnable functions transforming $|| \vec{r}_{ij} ||$ into weights of tensor products~\cite{schnet, nequip}. %:
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-3mm}
%\begin{equation}
%m_{ij} = f_j \otimes_{w(|| \vec{r}_{ij} ||)} \text{SH} \left( \frac{\vec{r}_{ij}}{|| \vec{r}_{ij} ||} \right)
%\label{eq:tensor_product_sh}
%\end{equation}
%where we use $w(|| \vec{r}_{ij} ||)$ to denote weights dependent on relative distance $||\vec{r}_{ij}||$~\cite{schnet}.
%%%Please refer to Sec.~\ref{appendix:subsec:tensor_product} in appendix for discussion on inversion in tensor products and Sec.~\ref{appendix:subsec:e3_qm9} and~\ref{appendix:subsec:e3_oc20} for additional results of including inversion.


% In order to interact different irrep features, we use the $O(3)$ tensor product.

% $SO(3)$ tensor products use Clebsch-Gordan coefficients, which are the expansion coefficients that project two irreps from different vector spaces onto the irrep basis in a single vector space. Intuitively, given two irreps of angular frequency $L_1$ and $L_2$ the $SO(3)$ tensor product expresses what are the possible total angular frequencies of the combined signal.

% The Clebsch-Gordan coefficients for $SO(3)$ are computed from integrals over the basis functions of a given irreducible representation, e.g. the real spherical harmonics, and are tabulated to avoid unnecessary computation.

% \begin{equation}
%     C_{(L_1, m_1) (L_2, m_2)}^{(L_3, m_3)} = \left|L_1 m_1; L_2 m_2 \right> \left<L_3 m_3 \right| = \int d{\Omega} Y^*_{L_1, m_1}(\Omega) Y^*_{L_2, m_2}(\Omega) Y_{L_3, m_3}(\Omega)
% \end{equation}

% For many combinations of $L_1$, $L_2$, and $L_3$ the Clebsch-Gordan coefficients are zero. The gives rise to the following selection rule for non-trivial coefficients: $-|L_1 + L_2| \lte L_3 \lte |L_1 + L_2|$.



% We call each distinct nontrivial combination of $L_1 \otimes L_2 \rightarrow L_3$ a path. For example, a vector ($L=1$, $p=-1$) tensor producted with a vector ($L=1$, $p=-1$) gives rise to three paths: a scalar ($L=0$, $p=1$), a pseudovector ($L=1$, $p=1$), and ($L=2$, $p=1$). Each path is independently equivariant, therefore we can further parameterize our tensor product with weights for each path \cite{e3nn}.

==> content/3_1_equivariant_operations.tex <==
\vspace{-2.5mm}
\subsection{Equivariant Operations for Irreps Features}
\vspace{-2.5mm}
\label{subsec:equivariant_operations}

%As irreps features encode directional and equivariant information in channel dimensions without complicating graph structures, we can adopt irreps features and inherit the design of existing networks through utilizing equivariant operations.
\revision{We discuss below equivariant operations, which serve as building blocks for equivariant graph attention and other modules, and analyze how they remain equivariant in Sec.~\ref{appendix:subsec:equivariant_operations}.}
%They include the equivariant version of the original operations in Transformers and the depth-wise tensor product, as illustrated in Fig.~\ref{fig:equivariant_operation} in appendix. %, an efficient version of tensor product.
They include the equivariant version of operations in Transformers and depth-wise tensor products as shown in Fig.~\ref{fig:equivariant_operation}. % in appendix. %, an efficient version of tensor product.

%\note{(We describe the difference of the operations in Equiformer from what has already introduced in Background.)}

%Since the internal representations are E(3) features, we replace the original operations with equivariant counterparts to preserve E(3)-equivariance and discuss equivariant versions of operations used in Transformer.
%Besides, we adopt the operation of tensor product to exchange the information contained in different type-$l$ vectors.

%\todo{Add figure for each of them!}

\vspace{-2.5mm}
\paragraph{Linear.}
Linear layers are generalized to irreps features by transforming different type-$L$ vectors separately.
Specifically, we apply separate linear operations to each group of type-$L$ vectors.
We remove bias terms for non-scalar features with $L > 0$ as biases do not depend on inputs, and therefore, including biases for type-$L$ vectors with $L > 0$ can break equivariance.
%Note that linear layers can be regarded as a special case of tensor product between E(3) features and type-$0$ constant one.

\vspace{-2.5mm}
\paragraph{Layer Normalization.}
Transformers adopt layer normalization (LN)~\citep{layer_norm} to stabilize training.
%\revision{
%Given input $x \in \mathbb{R}^{N \times C}$, with $N$ being the number of nodes and $C$ the number of channels, LN  calculates the linear transformation of normalized input as follows:
Given input $x \in \mathbb{R}^{N \times C}$, with $N$ being the number of nodes and $C$ the number of channels, LN  calculates the linear transformation of normalized input as $\text{LN}(x) = \left( \frac{  x - \mu_{C}  }{\sigma_{C}} \right) \circ \gamma + \beta$,
%\begin{equation}
%\text{LN}(x) = \frac{x - \mu_{C}}{\sigma_{C}} \circ \gamma + \beta
%\end{equation}
where $\mu_{C}, \sigma_{C} \in \mathbb{R}^{N \times 1}$ are mean and standard deviation of input $x$ along the channel dimension, $\gamma, \beta \in \mathbb{R}^{1 \times C}$ are learnable parameters, and $\circ$ denotes element-wise product.
%}
By viewing standard deviation as the root mean square value (RMS) of L2-norm of type-$L$ vectors, LN can be generalized to irreps features.
Specifically, given input $x \in \mathbb{R}^{N \times C \times (2L + 1)}$ of type-$L$ vectors, the output is
$\text{LN}(x) = \left( \frac{x}{\text{RMS}_{C}(\text{norm}(x))} \right) \circ \gamma$,
%\begin{equation}
%\text{LN}(x) = \frac{x}{\text{RMS}_{C}(\text{norm}(x))} \circ \gamma
%\end{equation}
where $\text{norm}(x) \in \mathbb{R}^{N \times C \times 1}$ calculates the L2-norm of each type-$L$ vectors in $x$, and $\text{RMS}_{C}(\text{norm}(x)) \in \mathbb{R}^{N \times 1 \times 1}$ calculates the RMS of L2-norm with mean taken along the channel dimension.
%%%We remove mean and biases for type-$L$ vectors with $L \neq 0$ following linear layers.
We remove means and biases for type-$L$ vectors with $L \neq 0$.

\vspace{-2.5mm}
\paragraph{Gate.}
We use the gate activation~\citep{3dsteerable} for equivariant activation function as shown in Fig.~\ref{fig:equivariant_operation}(c).
Typical activation functions are applied to type-$0$ vectors.
For vectors of higher $L$, we multiply them with non-linearly transformed type-$0$ vectors for equivariance.
Specifically, given input $x$ containing non-scalar $C_{L}$ type-$L$ vectors with $ 0 < L \leq L_{max}$ and $(C_0 + \sum_{L=1}^{L_{max}} C_L)$ type-$0$ vectors, we apply SiLU~\citep{silu, swish} to the first $C_0$ type-$0$ vectors and sigmoid function to the other $\sum_{L=1}^{L_{max}} C_L$ type-$0$ vectors to obtain non-linear weights and multiply each type-$L$ vector with corresponding non-linear weights.
After the gate activation, the number of channels for type-$0$ vectors is reduced to $C_0$.

\vspace{-2.5mm}
\paragraph{Depth-wise Tensor Product.}
The tensor product defines interaction between vectors of different $L$.
%%%To improve its efficiency, we use the depth-wise tensor product (DTP), which restricts one type-$L$ vector in output irreps features depends only on one type-$L'$ vector in input irreps features, where $L$ can be equal to or different from $L'$.
To improve its efficiency, we use the depth-wise tensor product (DTP), where one type-$L$ vector in output irreps features depends only on one type-$L'$ vector in input irreps features as illustrated in Fig.~\ref{fig:equivariant_operation}(d) and Fig.~\ref{fig:depthwise_tensor_product_e3nn}, with $L$ being equal to or different from $L'$.
This is similar to depth-wise convolution~\citep{mobilenet}, where one output channel depends on only one input channel. 
%, and therefore, we call it depth-wise tensor product (DTP).
Weights $w$ in the DTP can be input-independent or conditioned on relative distances, and the DTP between two tensors $x$ and $y$ is denoted as $x \otimes_{w}^{DTP} y$. % $x \tens_{w}^{DTP} y$.
%\todo{(Mention tensor product weights in Background)}
Note that the one-to-one dependence of channels can significantly reduce the number of weights and thus memory complexity when weights are conditioned on relative distances.
In contrast, if one output channel depends on all input channels, in our case, this can lead to out-of-memory errors when weights are parametrized by relative distances.

\begin{figure*}[t]
\includegraphics[width=0.85\linewidth]{figure/equivariant_operation.pdf}
\centering
\vspace{-3.5mm}
\caption{
\textbf{Equivariant operations used in Equiformer.}
%For ``Linear'', each gray line has one learnable weight.
\textbf{(a)} Each gray line between input and output irreps features contains one learnable weight.
%Note that the number of output channels can be different from that of input channels.
%The number of output channels can be different from that of input channels.
%For ``Layer Normalization'', ``RMS'' denotes root mean squared value with mean taken along channel dimension, and we remove multiplying by $\gamma$ in this figure for simplicity.  
%\textbf{(b)} ``RMS'' denotes the root mean square value (RMS) along the channel dimension.
\textbf{(b)} ``RMS'' denotes the root mean square value along the channel dimension.
For simplicity, we have removed multiplying by $\gamma$ here.
\textbf{(c)} Gate layers are equivariant activation functions where non-linearly transformed scalars are used to gate non-scalar irreps features.
\textbf{(d)} The left two irreps features correspond to two input irreps features, and the rightmost one is the output irreps feature.
%For ``Depth-wise Tensor Product'', the left two irreps features correspond to two input irreps features, and the rightmost one is output irreps feature.
The two gray lines connecting two vectors in the input irreps features and one vector in the output irreps feature form a path and contain one learnable weight.
An alternative visualization of depth-wise tensor products can be found in Fig.~\ref{fig:depthwise_tensor_product_e3nn} in appendix.
We show $SE(3)$-equivariant operations here, which can be generalized to $E(3)$-equivariant features.
}

\vspace{-4mm}
\label{fig:equivariant_operation}
\end{figure*}


==> content/5_1_qm9.tex <==
\vspace{-3mm}
\subsection{QM9}
\vspace{-3mm}
\label{subsec:qm9_exp}

\paragraph{Dataset.}
%%%The QM9~\citep{qm9_2, qm9_1} dataset (CC BY-NC SA 4.0 license) consisting of 134k small molecules, and the goal is to predict their quantum properties such as energy.
The QM9 dataset~\citep{qm9_2, qm9_1}  (CC BY-NC SA 4.0 license) consists of 134k small molecules, and the goal is to predict their quantum properties.
%The average number of atoms per molecule is 18, and each atom in a molecule comes from the set of H, C, N, O, F atoms and has 3D coordinates.
%%%We follow the data partition used by Cormorant~\cite{cormorant}, which has 100k, 18k and 13k molecules in training, validation and testing sets.
The data partition we use has 110k, 10k, and 11k molecules in training, validation and testing sets.
We minimize mean absolute error (MAE) between prediction and normalized ground truth. % and report MAE on the testing set.


\vspace{-3.25mm}
\paragraph{Training Details.}
Please refer to Sec.~\ref{appendix:subsec:qm9_training_details} in appendix for details on architecture, hyper-parameters and training time.


\vspace{-3.25mm}
\paragraph{Results.}
%%%We mainly compare with methods trained with the same data partition and summarize the results in Table~\ref{tab:qm9_result}.
We summarize the comparison to previous models in Table~\ref{tab:qm9_result}.
Equiformer achieves overall better results across 12 regression tasks compared to each individual model.
%%%Equiformer achieves the best results on 11 out of 12 tasks among models trained with same data partition.
The comparison to SEGNN, which uses irreps features as Equiformer, demonstrates the effectiveness of combining non-lienar message passing with MLP attention.
Additionally, Equiformer achieves better results for most tasks when compared to other equivariant Transformers, which are SE(3)-Transformer, TorchMD-NET and EQGAT.
This demonstrates a better adaption of Transformers to 3D graphs and the effectiveness of the proposed equivariant graph attention.
We note that for the tasks of $\mu$ and $R^2$, PaiNN and TorchMD-NET use different architectures, which take into account the property of the task.
%\revision{This makes the comparison less clear since we use the same architecture for all tasks.}
In contrast, we use the same architecture for all tasks.
We compare training time in Sec.~\ref{appendix:subsec:qm9_training_time_comparison}.

%%%Besides, the different data partition as denoted by $\dagger$ in Table~\ref{tab:qm9_result} has $10\%$ more molecules in the training set and less data in the testing set, and this can benefit some tasks that are more dependent on data partitions.
%\todo{If there is any justification, can write something like which tasks are more important.}

==> content/5_2_md17.tex <==
\begin{table}[t]
\begin{adjustwidth}{-2.5cm}{-2.5cm}
\centering
\scalebox{0.6}{
\begin{tabular}{lcccccccccccccccc}
\toprule[1.2pt]
                        & \multicolumn{2}{c}{Aspirin} & \multicolumn{2}{c}{Benzene} & \multicolumn{2}{c}{Ethanol} & \multicolumn{2}{c}{Malonaldehyde} & \multicolumn{2}{c}{Naphthalene} & \multicolumn{2}{c}{Salicylic acid} & \multicolumn{2}{c}{Toluene} & \multicolumn{2}{c}{Uracil} \\
\cmidrule[0.6pt]{2-17}
Methods                                               & energy       & forces       & energy       & forces       & energy       & forces       & energy          & forces          & energy         & forces         & energy           & forces          & energy       & forces       & energy       & forces      \\
\midrule[1.2pt]
SchNet~\citep{schnet}                          & 16.0         & 58.5         & 3.5          & 13.4         & 3.5          & 16.9         & 5.6             & 28.6            & 6.9            & 25.2           & 8.7              & 36.9            & 5.2          & 24.7         & 6.1          & 24.3        \\
DimeNet~\citep{dimenet}                          & 8.8          & 21.6         & 3.4          & 8.1          & 2.8          & 10.0         & 4.5             & 16.6            & 5.3            & 9.3            & 5.8              & 16.2            & 4.4          & 9.4          & 5.0          & 13.1        \\
PaiNN~\citep{painn}                                                 & 6.9          & 14.7         & -            & -            & 2.7          & 9.7          & 3.9             & 13.8            & 5.0            & 3.3            & 4.9              & 8.5             & 4.1          & 4.1          & 4.5          & 6.0         \\
TorchMD-NET~\citep{torchmd_net}                                           & \textbf{5.3}          & 11.0         & 2.5          & 8.5          & 2.3          & 4.7          & 3.3             & 7.3             & \textbf{3.7}            & 2.6            & \textbf{4.0}              & 5.6             & \textbf{3.2}          & 2.9          & \textbf{4.1}          & 4.1         \\
NequIP ($L_{max} = 3$)~\citep{nequip}                              & 5.7          & 8.0          & -            & -            & \textbf{2.2}          & 3.1          & 3.3             & 5.6             & 4.9            & \textbf{1.7}            & 4.6              & \textbf{3.9}             & 4.0          & \textbf{2.0}          & 4.5          & \textbf{3.3}         \\

\midrule[0.6pt]

Equiformer ($L_{max} = 2$)                                           & \textbf{5.3}          & 7.2          & \textbf{2.2}          & \textbf{6.6}          & \textbf{2.2}          & 3.1          & 3.3             & 5.8             & \textbf{3.7}            & 2.1           & 4.5              & 4.1             & 3.8          & 2.1          & 4.3          & \textbf{3.3}        \\
Equiformer ($L_{max} = 3$)                                           & \textbf{5.3}          & \textbf{6.6}          & 2.5          & 8.1          & \textbf{2.2}          & \textbf{2.9}          & \textbf{3.2}             & \textbf{5.4}             & 4.4            & 2.0           & 4.3              & \textbf{3.9}            & 3.7          & 2.1         & 4.3          & 3.4        \\
\bottomrule[1.2pt]
\end{tabular}
}
\end{adjustwidth}
\vspace{-3mm}
\caption{\textbf{MAE results on MD17 testing set.} Energy and force are in units of meV and meV/$\angstrom$.}
\vspace{-5.5mm}
\label{tab:md17_result}
\end{table}

\vspace{-3mm}
\subsection{MD17}
\vspace{-3mm}
\label{subsec:md17}


\paragraph{Dataset.}
The MD17 dataset~\citep{md17_1, md17_2, md17_3} (CC BY-NC) consists of molecular dynamics simulations of small organic molecules, and the goal is to predict their energy and forces.
We use $950$ and $50$ different configurations for training and validation sets and the rest for the testing set.
Forces are derived as the negative gradient of energy with respect to atomic positions. 
We minimize MAE between prediction and normalized ground truth.

\vspace{-3.25mm}
\paragraph{Training Details.}
Please refer to Sec.~\ref{appendix:subsec:md17_training_details} in appendix for details on architecture, hyper-parameters and training time.


\vspace{-3.25mm}
\paragraph{Results.}
We train Equiformer with $L_{max} = 2 \text{ and } 3$ and summarize the results in Table~\ref{tab:md17_result}.
Equiformer achieves overall better results across 8 molecules compared to each individual model.
%%%\revision{Compared to TorchMD-NET, which is also an equivariant Transformer, Equiformer obtains better MAE results.} 
%since the proposed equivariant graph attention is more expressive and can support vectors of higher degree $L$ (i.e., we use $L_{max} = 2$) instead of restricting to type-$0$ and type-$1$ vectors (i.e., $L_{max} = 1$).}
%%%\revision{The difference lies in the proposed equivariant graph attention, which is more expressive and can support vectors of higher degree $L$ (i.e., we use $L_{max} = 2 \text{ and } 3$) instead of restricting to type-$0$ and type-$1$ vectors (i.e., $L_{max} = 1$).}
Compared to TorchMD-NET, which is also an equivariant Transformer, the difference lies in the proposed equivariant graph attention, which is more expressive and can support vectors of higher degree $L$ (i.e., we use $L_{max} = 2 \text{ and } 3$) instead of restricting to type-$0$ and type-$1$ vectors (i.e., $L_{max} = 1$).
For the last three molecules, although Equiformer with $L_{max} = 2$ achieves lower force MAE but higher energy MAE, we can adjust the weights of energy loss and force loss so that Equiformer achieves lower MAE for both energy and forces as shown in Table~\ref{appendix:tab:md17_torchmdnet} in appendix.
%%%\revision{Compared to NequIP, which also uses irreps features and $L_{max} = 3$, Equiformer with $L_{max} = 2$ achieves overall lower MAE although including higher $L_{max}$ can improve performance and Equiformer uses smaller $L_{max}$.}
Compared to NequIP, which also uses irreps features and $L_{max} = 3$, Equiformer with $L_{max} = 2$ achieves overall lower MAE although including higher $L_{max}$ can improve performance.
When using $L_{max} = 3$, Equiformer achieves lower MAE results for most molecules.
This suggests that the proposed attention can improve upon linear messages even when the size of training sets becomes small.
We compare the training time of NequIP and Equiformer in Sec.~\ref{appendix:subsec:md17_training_time_comparison}.
Additionally, for Equiformer, increasing $L_{max}$ from $2$ to $3$ improves MAE for most molecules except benzene, which results from overfitting.

%\todo{[Training time of NequIP]}
%\todo{[Equiformer with $L_{max} = 3$]}

==> content/5_4_ablation_study.tex <==
\vspace{-2mm}

\begin{table}[t]
\centering
\scalebox{0.6}{

\begin{tabular}{cccclcccccccccc}
\toprule[1.2pt]
& \multicolumn{3}{c}{Methods} & & \\
\cmidrule[0.6pt]{2-4}
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non-linear \\ message passing\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MLP \\ attention\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dot product \\ attention\end{tabular}} &  Task & $\alpha$ & $\Delta \varepsilon$ & $\varepsilon_{\text{HOMO}}$ & $\varepsilon_{\text{LUMO}}$ & $\mu$ & $C_{\nu}$ & & Training time & Number of \\
%Index & & & & Unit & bohr$^3$ & meV & meV & meV & D & cal/mol K & & (minutes/epoch) & parameters \\
Index & & & & Unit & $a_0^3$ & meV & meV & meV & D & cal/mol K & & (minutes/epoch) & parameters \\
\midrule[1.2pt]

1 & \ding{51} & \ding{51} &  & & .046 & 30 & 15 & 14 & .011 & .023 & & 12.1 & 3.53M \\
2 & & \ding{51} &   & & .051 & 32 & 16 & 16 & .013 & .025 & & 7.2 & 3.01M \\
3 & & & \ding{51} & & .053 & 32 & 17 & 16 & .013 & .025 & & 7.8 & 3.35M \\
%4 & & \ding{51} &  &  & & .060 &  & 18 & 17 & .016 &  \\

\bottomrule[1.2pt]

\end{tabular}
}
\vspace{-3mm}
\caption{\textbf{Ablation study results on QM9.}}
\vspace{-3.25mm}
\label{tab:qm9_ablation}
\end{table}


\begin{table}[t]
\begin{adjustwidth}{-5 cm}{-5 cm}
\centering
\scalebox{0.6}{

\begin{tabular}{cccccccccccccccccc}
\toprule[1.2pt]
& \multicolumn{3}{c}{Methods} & & \multicolumn{5}{c}{Energy MAE (eV) $\downarrow$} & & \multicolumn{5}{c}{EwT (\%) $\uparrow$} \\
\cmidrule[0.6pt]{2-4}
\cmidrule[0.6pt]{6-10}
\cmidrule[0.6pt]{12-16}
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non-linear \\ message passing\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MLP \\ attention\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dot product \\ attention\end{tabular}} & & & & & & & & & & & & & Training time & Number of \\

Index & & & &  & ID & OOD Ads & OOD Cat & OOD Both & Average & & ID & OOD Ads & OOD Cat & OOD Both & Average & (minutes/epoch) & parameters \\
\midrule[1.2pt]

1 & \ding{51} & \ding{51} &  & & 0.5088 & 0.6271 & 0.5051 & 0.5545 &  0.5489  & & 4.88 & 2.93 & 4.92 & 2.98 & 3.93 & 130.8 & 9.12M \\
2 & & \ding{51} &   & & 0.5168 & 0.6308 & 0.5088 & 0.5657 & 0.5555 &  & 4.59 & 2.82 & 4.79 & 3.02 & 3.81 & 91.2 & 7.84M \\
3 & & & \ding{51}  & & 0.5386 & 0.6382 & 0.5297 & 0.5692 & 0.5689 & & 4.37 & 2.60 & 4.36 & 2.86 & 3.55 & 99.3 & 8.72M \\
%4 & & \ding{51} &  &  & 0.5213 & 0.6268 & 0.5178 & 0.5621 & 0.5579\\

%\bottomrule[1.2pt]
%\bottomrule[1.2pt]
%\vspace{-1mm}
%\\
%\toprule[1.2pt]

%%%\midrule[1.2pt]
%%%& \multicolumn{3}{c}{Methods} & & \multicolumn{5}{c}{EwT (\%) $\uparrow$} \\
%%%\cmidrule[0.6pt]{2-4}
%%%\cmidrule[0.6pt]{6-10}
%%%& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non-linear \\ message passing\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MLP \\ attention\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dot product \\ attention\end{tabular}} &  \\

%%%Index & & & & & ID & OOD Ads & OOD Cat & OOD Both & Average \\
%%%\midrule[1.2pt]

%%%1 & \ding{51} & \ding{51} & & & 4.88 & 2.93 & 4.92 & 2.98 & 3.93 \\
%%%2 & & \ding{51} &   &  & 4.59 & 2.82 & 4.79 & 3.02 & 3.81  \\
%%%3 & & & \ding{51} & & 4.37 & 2.60 & 4.36 & 2.86 & 3.55 \\
%4 & & \ding{51} &  &  & 4.37 & 2.80 & 4.40 & 2.98 & 3.64 \\

\bottomrule[1.2pt]

\end{tabular}
}

\vspace{-3mm}
\end{adjustwidth}
\caption{\textbf{Ablation study results on OC20 IS2RE validation set.}
%\note{Dot product attention uses smaller learning rate $1.5 \times 10^{-3}$.}
}
\vspace{-6.75mm}
\label{tab:oc20_ablation}
\end{table}



\vspace{-2.25mm}
\subsection{Ablation Study}
\vspace{-2.5mm} 
\label{subsec:ablation_study}

We conduct ablation studies \revision{to show that Equiformer with dot product attention and linear message passing has already achieved strong empirical results and demonstrate} the improvement brought by MLP attention and non-linear messages in the proposed equivariant graph attention.
%We modify dot product (DP) attention~\citep{transformer, se3_transformer} so that it only differs from MLP attention in how attention weights $a_{ij}$ are generated from $f_{ij}$.
\revision{Dot product (DP) attention only differs from MLP attention in how attention weights $a_{ij}$ are generated from $f_{ij}$.}
%%%Please refer to Sec.~\ref{appendix:subsec:dot_product_attention} in appendix for details on DP attention.
Please refer to Sec.~\ref{appendix:subsec:dot_product_attention} in appendix for further details.
For experiments on QM9 and OC20, unless otherwise stated, we follow the hyper-parameters used in previous experiments. 
%\revision{Please refer to Sec.~\ref{appendix:subsec:qm9_training_details} and Sec.~\ref{appendix:subsec:oc20_training_details} for training time of different models.}

\vspace{-3.25mm}
\paragraph{Result on QM9.}
The comparison is summarized in Table~\ref{tab:qm9_ablation}.
\revision{Compared with models in Table~\ref{tab:qm9_result}, Equiformer with dot product attention and linear message passing (Index 3) achieves competitve results.}
%Non-linear messages improve upon linear messages when MLP attention is used.
Non-linear messages improve upon linear messages when MLP attention is used while non-linear messages increase the number of tensor product operations in each block from $1$ to $2$ and thus inevitably increase training time.
%%%Similar to what is reported by GATv2~\cite{gatv2}, the improvement of replacing DP attention with MLP attention is not very significant.
%%%\todo{On the other hand, the improvement of replacing DP attention with MLP attention is not very significant.}
On the other hand, MLP attention achieves similar results to DP  attention.
We conjecture that DP attention with linear operations is expressive enough to capture common attention patterns as the numbers of nighboring nodes and atom species are much smaller than those in OC20.
However, MLP attention is roughly $8\%$ faster as it directly generates scalar features and attention weights from $f_{ij}$ instead of producing additional key and query irreps features for attention weights.

\vspace{-3.25mm}
\paragraph{Result on OC20.}
%%%We consider the setting of training without IS2RS auxiliary task and use a smaller learning rate $1.5 \times 10 ^{-4}$ for DP attention as this improves the performance.
We consider the setting of training without auxiliary task and summarize the comparison in Table~\ref{tab:oc20_ablation}.
%%%We summarize the comparison in Table~\ref{tab:oc20_ablation}.
\revision{Compared with models in Table~\ref{tab:is2re_validation}, Equiformer with dot product attention and linear message passing (Index 3) has already outperformed all previous models.}
Non-linear messages consistently improve upon linear messages.
In contrast to the results on QM9, MLP attention achieves better performance than DP attention and is $8\%$ faster.
We surmise this is because OC20 contains larger atomistic graphs with more diverse atom species and therefore requires more expressive attention mechanisms.
Note that Equiformer can potentially improve upon previous equivariant Transformers~\citep{se3_transformer, torchmd_net, eqgat} since they use less expressive attention mechanisms similar to Index 3 in Table~\ref{tab:oc20_ablation}.

==> content/7_checklist.tex <==

\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include code related to experiments on QM9 in supplementary. Code reproducing all experiments will be available.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{As each experiment takes much time, we are not able to run several times. However, the proposed method improves upon previous works by a clear margin, and therefore the improvement is not within noise ranges.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> content/8_4_broader_impacts.tex <==
\section{Broader Impacts}
\label{appendix:sec:broader_impacts}

